Sparsification as a Remedy for Staleness in Distributed Asynchronous SGD

Large scale machine learning is increasingly relying on distributed optimization, whereby several machines contribute to the training process of a statistical model. In this work we study the performance of asynchronous, distributed settings, when applying sparsification, a technique used to reduce communication overheads. In particular, for the first time in an asynchronous, non-convex setting, we theoretically prove that, in presence of staleness, sparsification does not harm SGD performance: the ergodic convergence rate matches the known result of standard SGD, that is $\mathcal{O} \left( 1/\sqrt{T} \right)$. We also carry out an empirical study to complement our theory, and confirm that the effects of sparsification on the convergence rate are negligible, when compared to 'vanilla' SGD, even in the challenging scenario of an asynchronous, distributed system.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> src/practical.tex <==
{\color{red}
In this Section, we could give an alternative, practical view on sparsification.
This is where we could introduce what will be later shown in the experiments:
\begin{itemize}
    \item Sparsification can be seen as different learning rates applied to parameter elements, depending on their importance
    \item We could also argue about the \texttt{rand} operator
    \item Eventually, if we find a connection to pre-conditioning, this is also a place to discuss it
\end{itemize}
}

==> src/related.tex <==
\subsection{Asynchronous SGD}

\paragraph{}
In~\cite{Damaskinos:2018}, the authors address two problems: Byzantine fault tolerance and asynchrony.
The main idea is to define a ``cone'' of ``acceptable'' gradient updates, that is those gradients that are
not too far off the average gradient direction.
In addition, to combat staleness due to asynchrony, gradient updates are weighted by a damping function that
attenuates the contribution of stale gradients.

The underlying parameter server model is underspecified: a single master receives updates, accumulates $M$
of them in an update sequence, then broadcasts the update to all workers.
It is unclear if workers block upon a parameter update and start over or not.

Convergence and convergence rate proofs follow mainly~\cite{Bottou:2018}: if gradient updates are within the
``cone'' and other assumptions on Lispshitness of the gradients and bounded variance of the loss function,
the modified update rule converges at a rate proportional to $1/\sqrt{T}$, in spite of $f$ Byzantine workers.
{\color{red}Need to check about emphasis on staleness values.}

Experiments validate the damping function, not Byzantiness, and use an unknown simulator.
\begin{itemize}
    \item Metrics used: cost and accuracy per epoch / model update.
    \item Parameters explored: staleness: Gaussian distribution; workers = 10.
    \item Models: Simple CNN on CIFAR-100.
    \item Competitors: naive asynchronous SGD, ideal synchronous SGD~\cite{Jiang:2017}.
\end{itemize}
Main results:
\begin{itemize}
    \item ASGD does not converge, with mean staleness of 12
    \item Kardam vs.~\cite{Jiang:2017} difference is negligible $\to$ don't dampen too much stale updates
    \item Increasing average staleness decreases convergence rate, as from theory
\end{itemize}

\paragraph{}
In~\cite{Dai:2018}, the authors aim at clarifying the statistical efficiency system throughput trade-off that underlies
the parameter server architecture, under a controlled delayed scenario.
First, the authors discuss the findings of a large simulation campaign, where they use an atypical parameter server
architecture: each worker broadcasts its gradients to all other workers, who then use all received updates to compute
the new model.
Note that the simulator is not available.
Depending on the delay distribution (which is assumed to be categorical), messages might not arrive in time for a model
update to include all contributions.
In their simulation they go beyond training deep neural network models, and also study matrix factorization,
topic modeling and variational autoencoders.
Furthermore, they study the impact of variants of the baseline gradient descent algorithm, including momentum, adam,
adagrad and RMSprop.
In terms of datasets, they use the typical ones: e.g. for classification they use CIFAR-100 and MNIST.

Experimental methodology:
\begin{itemize}
    \item Metrics used: number of batches (i.e., model updates) to reach a given accuracy (71\%); they also
    introduce a normalization factor to base results on no-staleness; cosine similarity as a function of
    number of batches
    \item Parameters explored: staleness: categorical distribution; number of workers: $\{1, 8, 16\}$
    \item Models: DNN, CNN, VAE on CIFAR-100, MNIST
    \item Competitors: none
\end{itemize}
Main results:
\begin{itemize}
    \item Convergence under higher level of staleness requires more batches to be processed in order to
    reach the same model quality. From Fig.1 in~\cite{Dai:2018}, this is especially true for the Adam optimizer,
    but not so much for SGD. Note also, that this results is for 8 workers. The consequence for the authors is:
    if the slowdown due to asynchrony is too high, use staleness minimization system designs or synchronous
    execution
    \item The staleness level acceptable in distributed training can depend strongly on the complexity of the model.
    For sufficiently complex models it may be more advantageous to eliminate staleness altogether and use
    synchronous training.
    \item Algorithm sensitivity to staleness: here we compare variants of gradient descent, and we vary the number of
    workers. Overall, SGD seems more robust to staleness, whereas adam, momentum and RSMProp suffer severely from
    staleness. One important observation from Fig.2 in~\cite{Dai:2018} is that there is apparently no speedup
    whatsoever when increasing the number of workers: scalability seem to be very bad.
\end{itemize}

From the theory point of view, the authors in~\cite{Dai:2018} introduce the concept of \emph{gradient coherence}:
formally this is the minimum angle between gradients at the current iteration and all previous gradients within a
window of $s$ time-stamps in the past.
If the coherence is positive, then current gradients are aligned with past ones.
In this case, the convergence property induced by using delayed stochastic gradients is close to that induced by
using synchronous stochastic gradients.
Note that gradient coherence can be easily estimated at runtime.
Using gradient coherence, they suggest a learning rate that is: proportional to gradient coherence, and inversely
proportional to the staleness level (and the number of updates within the staleness level, which is a function of
the number of workers.)
Convergence and convergence rates are proven under the assumptions of: a loss function that is continuously
differentiable and bounded by below, and Lipshitz continuous gradients of the loss.

\paragraph{}
In~\cite{Lian:2015:APS:2969442.2969545} authors study the asynchronous parallel stochastic gradient algorithm for nonconvex optimization.
Mathematical assumptions: unbiased gradient, bounded variance, lipschitzian gradient, independent samples, bounded staleness. Notation: M workers, K iterations.
They consider two implementations: consistent (AsySG-con) and inconsistent (AsySG-incon) asynchronous parallel SG. The first one is over a computer network, which ensures atomicity of reading and writing the whole vector of parameters; the second one is on a shared memory system, which only ensures efficiency for atomic reading and writing on a single coordinate of the parameter vector, thus leading to an inconconsistent parameter state. For both algorithms the convergence rate is proved to be $\mathcal{O}(1/\sqrt{MK})$, thus a linear speedup is achieved if M is bounded by $\mathcal{O}(\sqrt{K/M})$.

Experimental methodology:
\begin{itemize}
    \item Metrics: iteration speedup of T workers wrt serial SG (one worker), running time speedup wrt serial SG
    \item Parameters: number of workers from 1 to 8, number of cores from 1 to 32
    \item Models: AsySG-con: LeNet on MNIST, CIFAR10-FULL on CIFAR-10; AsySG-incon: Deep neural network for synthetic data
\end{itemize}

Main results:
\begin{itemize}
    \item Iteration speedup is always better than running time speedup
    \item Time speedup for CIFAR10-FULL is slightly more stable than LeNet, which has more parameters and thus requires more communication cost 
    \item Overall performance of AsySG-incon on the shared memory system is better than AsySG-con on the computer cluster, due to: computer cluster suffers from serious communication delay, delay bound on computer cluster is usually larger than on shared memory system
\end{itemize}

\paragraph{}
In~\cite{pmlr-v84-dutta18a} authors present a theoretical analysis of the trade-off between the error and the actual runtime (instead of iterations), for different variants of SGD. They also propose a new learning rate schedule to compensate for staleness and stabilize asynchronous SGD. 
The distributed architecture is the classical PS-workers, but they consider four different variants of SGD:

\begin{itemize}
    \item K-sync SGD: this is the synchronous scheme introduced by \cite{45187}, in which the PS only waits for the first K out of P learners to push their gradients.
    \item K-batch-sync: all the P learners start computing gradients with the same parameters; whenever any learner finishes, it pushes its update to the PS and evaluates the gradient on the next mini-batch with the same parameters; the PS updates using the first K mini-batches that finish and cancels the remaining learners. K-batch-sync offers advantages over K-sync in runtime as no learner is idle.
    \item K-async SGD: all the P learners compute their gradients on a single mini-batch. The PS waits for the first K out of P that finish first, but it does not cancel the remaining learners. Thus, for every update the gradients returned by each learner might be computed at a stale or older value of the parameter.
    \item K-batch-async: the PS waits for K mini-batches before updating itself but irrespective of which learner they come from; so wherever any learner finishes, it pushes its gradient to the PS, fetches current parameters at PS and starts computing gradient on the next mini-batch based on the current values of the PS. Again this version reduces runtime as no learner is idle.
\end{itemize}

Under the assumptions introduced in \cite{Bottou:2018} of Lipschitz-continuous gradient, unbiased stochastic gradient, bounded variance, they prove the speed up offered by asynchronous over synchronous SGD and by K-batch-async over K-async, using different distributions for the random variables representing the wall clock time of each learner to process a single mini-batch.
In the convergence analysis, instead, they relax some assumptions of the existing literature and they prove that async-SGD has faster decay with time but a higher error floor, while K-batch-async gives intermediate performance between async and sync-SGD. These main results are proved for strongly convex objective functions, but they expand also the analysis to obtain weaker guarantees for non-convex objectives.
For the learning rate schedule, they propose to weigh more a gradient if it is less stale and scale down its contribution otherwise. This schedule gives fast convergence and also maintains stability for async-SGD.

\begin{itemize}
    \item Parameters: number of workers to wait: \{2,4,8\}, mini-batch: \{256, 1024, 2048\}
    \item Models: single layer network on MNIST and CIFAR-10 with 8 workers, Alexnet on ImageNet with 4 workers
\end{itemize}

\paragraph{}
In \cite{Simsekli:2018} the authors work on second order methods, and more precisely on L-BFGS, which uses an approximate
Hessian and additional techniques to mitigate space complexity of the algorithm.
In this work, the authors draw parallels between optimization and Markov Chain Monte Carlo (MCMC) techniques for sampling
from a posterior distribution, thanks to the addition in the problem formulation of an Gaussian noise (which also allows
excaping from local minima).
The base architecture is that of a simple parameter server in an \emph{asynchronous} setting: a single master aggregates
contributions from workers, which can access all data samples and process them independently.
In addition, the authors introduce momentum, which helps with algorithm stability.

The authors provide non-asymptotic proofs of convergence and covergence rate.
In particular, they first develop a continuous-time Markov process whose marginal stationary measure admits a density
that is proportional to a function of the loss.
Then they show that the proposed algorithm forms an approximate Euler-Maruyama integrator that approximately simulates
the continuous process in discrete-time.
Finally, they analyze this approximate numerical scheme and provide a non-asymptotic error bound on the ``divergence''
or ergodic error between the approximate loss and the optimal loss.
They do that by decomposing it in two terms: the first accounts for the bias of the statistical estimator, and the
second has to be bounded using arguments on bounds on the variance.
All proofs assume Lipshitz continuity and bounded variance.

From the experimental point of view, results are quite limited, although they develop both a MATLAB simulator, and
a real implementation based on MPI.

Experimental methodology:
\begin{itemize}
    \item Metrics: Gradient norms, RMSE, time to converge
    \item Parameters: Number of workers
    \item Models: Matrix factorization
    \item Competitors: Asynchronous SGD
\end{itemize}

Main results:
\begin{itemize}
    \item AS-L-BFGS converges slightly faster than A-SGD
    \item AS-L-BFGS is substantially better than mini-batch L-BFGS
    \item AS-L-BFGS has an approximately linear speed-up with the number of workers
\end{itemize}

\subsection{Stale Synchronous Parallel (SSP)}

In~\cite{Jiang:2017}, the authors study the stale-synchronous model (SSP) first presented in~\cite{Ho:2013}, in the
context of an heterogeneous parameter server architecture.
Note that the SSP model is somehow different from the model we use: each worker has a local model; updates from workers
to the parameter server involve models, not gradients; the parameter server averages models, not gradients; workers
update the local model with the global one, if some conditions apply (see also a more detailed review
about~\cite{Ho:2013}).

The heterogeneity among workers induces staleness, which the authors address by operating on the learning rates used
by the SSP parameter server architecture.
Formally, the heterogeneity of the cluster is measured by the speed gap between the fastest worker and the slowest
worker.

The first contribution of the paper is to study, in a real cluster, the anatomy of existing systems: \emph{i)} BSP model,
that is synchronous SGD, in the presence of stragglers, the overall processing time is determined by the slowest
worker; \emph{ii)} ASP model, that is completely asynchronous SGD, is often faster than BSP systems in homogeneous clusters,
but when some stragglers are significantly slower than other machines, ASP cannot guarantee correct convergence;
\emph{iii)} SSP model, in heterogeneous environments, the global parameter and the replica of a straggler can be
inconsistent, thus the update generated by a straggler might push the global parameter to some place distant from
the optimality at a time when the global parameter is already near the optimality.

The second contribution of the paper is to propose two variants of the SSP model, in which the global learning rate,
that is the learning rate used by the parameter server, is used to ``dampen'' the contribution of stale workers.
The two variants differ in that in the baseline, we have one global learning rate across workers, whereas in the
extended version, each worker is applied a different learning rate that takes into account staleness.
The theoretical proofs of convergence rely on a ``regret minimization argument''.
Convergence rate is as usual $1/\sqrt{T}$, and the constants are: proportional to the square root of the staleness and
to the number of workers to the power of 1.5.\footnote{Note that this is in contrast to the constants used
in~\cite{Dai:2018}.}

Experimental methodology:
\begin{itemize}
    \item Metrics used: wall-clock time to convergence to a target accuracy; number of parameter server updates to
    reach a given accuracy; time per parameter update;
    \item Parameters explored: staleness, this is an important parameter of their algorithm, as for SSP
    \item Models: logistic regression, SVM, on URL and a proprietary dataset
    \item Competitors: BSP: Spark, TensorFlow; ASP: TensorFlow; SSP: Petuum
\end{itemize}

\subsection{Synchronous SGD}

\paragraph{}
In~\cite{Chen:2018:FDD:3267809.3275463} the authors propose a new synchronization
scheme called LB-BSP (Load-balanced BSP). The idea is to eliminate stragglers by adapting workers training load to their processing capability; that is, slower workers receive a smaller batch of data to process.
The considered distributed setup regards non-dedicated clusters, where workers computational capabilities can be highly different and stragglers are non-transient and salient, differently from dedicated clusters, where all workers have similar computation capabilities and stragglers are transient.
They describe the main existing coordinating schemes, i.e. BSP, ASP, SSP~\cite{Ho:2013}, DynSSP~\cite{Jiang:2017}, comparing them in terms of hardware efficiency and statistical efficiency. Then they justify the choice of the worker-adaptive batch sizing solution, listing four properties of deep learning workloads (short iterations, strong iterative-ness, load inner-homogeneity, load indivisibility), which make inefficient the existing load balancing approaches.

The basic intuition of LB-BSP is to adaptively adjust the batch size of each worker so as to equalize their batch processing times, defined as the composition of computation time and communication time. They hence solve an optimization problem, distinguishing the case of CPU- and GPU-clusters. In the first ones, the batch processing time depends on the sample processing speed, which they predict using the NARX model with input the speed, CPU and memory at previous iterations. In the second ones, the relation between computation time and batch size is more complicated, thus they describe it doing an offline profiling of the GPU performance. This accomplishes the goal of achieving the best hardware efficiency as ASP.
To achieve also statistical efficiency, they propose to weight a worker's gradient using its batch size, in the aggregation phase.

Experimental methodology:
\begin{itemize}
    \item Metrics: number of updates PS receives until model converges, per-update time, total run time, resources wastage (measured as average percentage of iteration time spent by workers waiting), overhead caused by log processing and batch size updating
    \item Parameters: heterogeneity level (in terms of straggler's speed), cluster configuration: {32 workers, 8 GPUs}
    \item Models: ResNet-32 on CIFAR-10, Inception-V3 on ImageNet
    \item Competitors: BSP, ASP, SSP with Tensorflow (CPU-cluster) and MXNet (GPU-cluster)
\end{itemize}

Main results:
\begin{itemize}
    \item LB-BSP requires the same number of updates for convergence as BSP and it shares similar average iteration time with ASP; it outperforms the other schemes in case of high heterogeneity
    \item SSP and BSP have similar performance when stragglers are non-transient
\end{itemize}

\paragraph{}
In~\cite{NIPS2018_7874} authors use the idea, proposed by \cite{45187}, of mitigating the stragglers' effect by setting a threshold for the number of workers on which to wait before synchronously updating the parameter on the PS, but improve the way the likely number of stragglers is identified, thus obtaining a cutoff that evolves dynamically with the iterations.
The proposed algorithm, called Bayesian distributed SGD (BDSGD), consists in predicting the joint run-time behavior of all workers and using this to set the optimal choice of straggler cutoff that maximizes gradient computation throughput.
Worker run-times are modeled with a deep state space model, where transition and emission functions are parameterized by neural networks, and training is performed using amortized inference, which enables real-time predictions.

Experimental methodology:
\begin{itemize}
    \item Metrics: throughput (parameter updates per unit time), cutoff (number of workers to wait for), training time, wall clock time saved over naive synchronous SGD
    \item Parameters: number of workers: {158, 2175}
    \item Models: 2-layer CNN on MNIST and ResNet-16, ResNet-64, and WideResNet-16x10 on CIFAR-10
    \item Competitors: asynchronous SGD (Hogwild), synchronous SGD, Chen et al. \cite{45187}
\end{itemize}

Main results:
\begin{itemize}
    \item BDSGD achieves the fastest convergence to the lowest loss
    \item BDSGD predicts the best cutoff that leads to the highest throughput
\end{itemize}

\subsection{Local SGD}

\paragraph{}
In \cite{Lin:2018} the authors advocate for another variant of SGD, that is called \emph{local SGD}.
In the literature, this approach is well known and also goes under the name of Iterative Parameter Mixing.
In a nutshell, with local SGD every worker maintains a local model, which is optimized using locally available
training data: each local model update is done using standard mini-batch SGD.
Then, once every several local update steps, workers propagate (either through a parameter server or by direct
communication) their local model for a global update step, which consists in some variants of model averaging.

The theoretical convergence properties of local SGD are only partially understood: as usual, stronger guarantees exist
for convex loss functions, weaker rates apply to non-convex functions.
Moreover, in this work (and appranetly in the literature) the focus is on \emph{synchronous} communications.
In this paper, the convergence rate is ``borrowed'' from other works in the literature, and is defined to be:
$\mathcal{O}(\frac{1}{\sqrt{T H K B_{loc}}})$

Why local SGD is supposed to work better?
Simply because we can ``modulate'' the number of global updates that are required, which implies fewer communication
steps, that are assumed to be the bottleneck.

Experimental methodology:
\begin{itemize}
    \item Metrics: accuracy vs. model updates; accuracy vs. time; accuracy vs. epochs; speedup vs. workers accuracy vs. workers
    \item Parameters: number of workers (i.e., number of GPUs); network delay
    \item Models: ResNet-20 on CIFAR 10/100 and ResNet-50 on ImageNet-1k, DenseNet and WideResNet. A lot of emphasis is put
    on model initialization and ``learning tricks''.
    Data is reshuffled at every epoch.
\end{itemize}

Main results:
\begin{itemize}
    \item Because local SGD requires less communication, it is faster to converge than mini-batch SGD
    \item Local SGD achieves better accuracy because it uses smaller batch size
    \item Local SGD scales almost linearly with the number of workers, again because of less communication
\end{itemize}

\paragraph{}
The work presented in \cite{Stich:2018} is the polished version of \cite{Lin:2018}, in which formal proofs of
convergence for Local SGD in the strongly convex settings are given.
The proof method is different than those based on \cite{Bottou:2018}, albeit there still is a concept of a converging
sequence.
Here the bound is given on the expected deviation of the loss function evaluated with the last iterate $T$, and the
optimal loss.
The proof outline follows perturbed iterate analysis, where worker series of updates are compared to an average
update.
This latter is the one that is used to compute the bounds of the expected deviation above.
In this work, the author also presents an asynchronous version of Local SGD, and uses similar arguments
used in the proofs of convergence in the synchronous case.
The author conjectures that convergence proofs for the non-convex case can simply follow those for the
strongly convex case.

The main take home message in \cite{Stich:2018} is that the convergence rate of Local SGD scales linearly with the
number of workers, which is achieved when the global update schedule follows a well defined ``horizon''
$H=\mathcal{O}(T / (K b))$.
This, essentially, means that we substantially limit the need for frequent global model synchronizations, which are the
main source of communication overheads.

\paragraph{}
In~\cite{Zhang2016ParallelSW} authors consider parallel SGD, where many workers compute their model parameters and at the update phase an average of the models is computed. They hence study the effect of performing one single average at the end of the training (one-shot averaging) or averaging the models after every iteration (mini-batch averaging). The idea is to use the averaging frequency to trade off statistical and hardware efficiency of the algorithm.
Through two examples of convex problems, they demonstrate that conventional modeling fails
to capture the empirical benefits of frequent averaging, that is variance reduction. Thus they propose a new model for gradient variance, which at every step depends on the distance from the optimum. In convex problems they empirically show that periodic averaging improves the convergence speed when the variance is higher far from the optimum. For non-convex problems, periodic averaging speeds up convergence significantly compared to one-shot averaging, due to the presence of different local minima, whose combination at the end leads to higher training loss.

\begin{itemize}
    \item Metrics: training loss, training and test error
    \item Parameters: frequency of averaging: \{one-shot, 128, 1024 iterations\}
    \item Models: least squares regression and logistic regression on a total of 5 datasets, 2-layer CNN with LeNet filters on MNIST
\end{itemize}

\paragraph{}
The work in~\cite{Yu2019ParallelRS} extends the theoretical analysis in \cite{Stich:2018} for non-convex optimization. The adopted approach is that of model averaging, where each worker maintains its local model and every I iterations it updates its local solution using an average model. They demonstrate that a linear speedup wrt the number of workers, i.e. $\mathcal{O}(\frac{1}{\sqrt{NT}})$, is achieved if the averaging interval $I=\mathcal{O}(\frac{T^{1/4}}{N^{3/4}})$, while reducing communication costs. The proof, although different from the usual ones, is well explained and the bound is given on the average expected squared gradient norm. Additionally, they extend the algorithm with time-varying learning rates, for the case where the time horizon $T$ is not known beforehand, and asynchronous SGD in heterogeneous networks. The latter is implemented by letting faster workers run more iterations than slower ones before model averaging.

Experimental methodology:
\begin{itemize}
    \item Metrics: training loss and test accuracy vs time
    \item Parameters: synchronization interval $I=\{4,8,16,32\}$
    \item Models: ResNet-20 on CIFAR-10
    \item Competitors: synchronous SGD, implemented with Horovod (all-reduce method, not PS)
\end{itemize}

\paragraph{}
In~\cite{ijcai2018-447} authors analyze a synchronous K-step averaging SGD (i.e. local SGD), by studying its convergence for non-convex objectives. The proof follows \cite{Bottou:2018}, whereby the bound is given on the average expected squared gradient norm, and the resulting convergence rate is $\mathcal{O}(\frac{\sqrt{K}}{\sqrt{NT}})$, that is the K-AVG algorithm loses a factor of $\frac{1}{\sqrt{K}}$ as a result of communication saving. However, they show that adopting diminishing stepsizes and/or dynamic batch sizes makes the expected average squared gradient norms converge to zero instead of a nonzero constant. Moreover, they show that K-AVG allows larger stepsizes than asynchronous SGD and that the former scales better with the number of workers than the latter. Finally they study the impact and optimal choice of K, indicating that when the solution is far away from the optimum, larger K (i.e. less frequent synchronizations and so larger variance) can lead to faster convergence rate.

Experimental methodology:
\begin{itemize}
    \item Metrics: test accuracy, speedup over competitors
    \item Parameters: number of workers: $\{8,16,32,64,128\}$, averaging frequency K: \{1,2,4,8,16,32,64\}
    \item Models: VGG and NIN on CIFAR-10
    \item Competitors: two asynchronous SGD implementations: \textit{Downpour}~\cite{NIPS2012_4687} and \textit{EAMSGD}~\cite{NIPS2015_5761}
\end{itemize}

\subsection{Sparsified SGD}

\paragraph{}
In~\cite{NIPS2018_7837} authors focus on gradient sparsification methods and prove that they provide convergence guarantees for SGD, with convex and non-convex objectives. Specifically, the TopK algorithm works as follows. Once a node has computed its local gradient, this is truncated to its top K components, sorted in decreasing order of magnitude, and sent to other nodes or to a PS. Additionally, the node accumulates locally the error resulting from the truncation; this error is always added to the current gradient before truncation. The convergence proof is based on the assumption, experimentally validated, that the gap between the sum of top-K components (as is the case of TopK algorithm) and the top-K of the gradient sum (which would be applied in a sequential version) is bounded. This assumption can be viewed then as a bound on the variance of the local gradients with respect to the global variance.

\begin{itemize}
    \item Metrics: error and training loss vs epoch
    \item Models: linear regression on synthetic data, logistic regression on RCV1, ResNet110 on CIFAR-10
    \item Competitors: Asynchronous SGD
\end{itemize}

Main results:
\begin{itemize}
    \item Convex-case: the gradient norm is concentrated towards the top elements. Non-convex case: $K=cn$ with $c>1/2$, in the worst-case of uniformly distributed gradients.
    \item Sparsification methods provide convergence guarantees because they implicitly maintain bounds on the maximum impact of stale updates
\end{itemize}

\paragraph{}
The work in~\cite{NIPS2018_7405} proposes to reduce the communication cost, by sparsifying the gradient and reducing its coding length. The sparsification technique consists in randomly dropping some coordinates of the stochastic gradient and appropriately amplifying the remaining coordinates to ensure the unbiasedness of the sparsified gradient. The algorithm is based on the idea that the convergence of SGD is significantly dominated by the variance of the gradient, thus they try to find the optimal trade-off between sparsity and variance, formulating it as a linear planning problem. The closed-form solution of the problem indicates that for several coordinates of the gradient the probability of keeping the value is 1, and for other coordinates the probability is proportional to the magnitude of the gradient. The sparsified gradient is then packed into a message with a particular coding strategy. They theoretically prove that when the distribution of gradient magnitude values is highly skewed, there is a significant gain in applying the proposed sparsification strategy.

Experimental methodology:
\begin{itemize}
    \item Metrics: convergence speed
    \item Parameters: sparsity of data points and gradients, number of workers (threads): \{16,32\}, learning rate
    \item Models: logistic regression on synthetic data, 3-layer CNN on CIFAR-10, multi-thread SVM on synthetic data
    \item Competitors: uniform sampling of gradient's coordinates, vanilla SGD, QSGD~\cite{NIPS2017_6768}
\end{itemize}

Main results:
\begin{itemize}
    \item With sparser data, the algorithm generates gradient with smaller variance and converges faster, consistently with the objective function
    \item With non-convex problems, the sparsification technique slows down the training efficiency only slightly and significantly reduces the communication cost
    \item With asynchronous SGD, gradient sparsification significantly reduces the conflicts among multiple threads for reading and writing the same coordinate, leading to a higher training speed. Moreover, it scales up with the number of threads
\end{itemize}

\paragraph{}
In~\cite{pmlr-v70-sun17c} authors propose \textit{meProp}, a minimal effort back propagation method. It is a general technique for neural network learning and not conceived for distributed approaches only. The idea is to reduce the computational cost of back propagation, by computing only a small subset of the full gradient to update model parameters. In particular, the gradient vectors are “quantized” so that only the top-k components in terms of magnitude are kept. They demonstrate that applying \textit{meProp} can substantially speed up the back propagation, as it provides a linear reduction in the computational cost. Moreover, updating only 1–4\% of the weights at each back propagation pass does not result in a larger number of training iterations and the model's accuracy is improved, rather than degraded. Their intuition is that the minimal effort update does not modify weakly relevant parameters, which makes overfitting less likely, similar to the dropout effect. Comparing with dropout technique, they find that \textit{meProp} can achieve further improvement, which suggests that the type of overfitting that \textit{meProp} reduces is probably different from that of dropout.

Experimental methodology:
\begin{itemize}
    \item Metrics: back propagation time, training time, accuracy
    \item Parameters: $k$, number of hidden layers
    \item Models: LSTM for NLP problem, MLP on MNIST
\end{itemize}

